Global Stability for Charged Scalar Fields in an Asymptotically Flat Metric in Harmonic Gauge

We prove global stability for the Charge-Scalar Field system on a background spacetime which is close to $1+3$-dimensional Minkowski space and whose outward light cones converge to those for the Schwarzschild metric at null infinity. The key technique to this proof is the use of a modified null frame, depending only on the mass $M$ of the metric, which captures the asymptotic behavior of the metric at future null infinity. Our results are analogous to results obtained in Minkowski space by Lindblad and Sterbenz up to a change in coordinates, and will in the sequel be used to prove the full structure of the Einstein-Charge scalar field system in these modified harmonic coordinates.

==> ChJuly/ChargeTermsDeleted.tex <==
We now look at the current. We do not have the identity $\overline{J}_{\Ls} = \overline{J}_{B_j^*} = 0$ as in the Minkowski case; however, for now we can treat all terms as equal to their Minkowski analogues plus an error term with nice decay scaling with $\epsilon$ (which may be bounded by the energy of the metric for high derivatives), as usual. For the case where $J$ is undifferentiated, we can establish nice estimates on components.
We define these here:

\begin{equation}
\nabla^\beta \overline{F}_{\alpha\beta} = g^{\beta\gamma}\partial_\gamma \overline{F}_{\alpha\beta} - \overline{F}^{\sigma\gamma}\partial_\gamma g_{\alpha\sigma},
\end{equation}
where the simplification follows from the harmonic gauge and antisymmetry of $F$. We see that, as in the Minkowski case, $\overline{J}_{\uLs}$ appears even in the Minkowski case and scales with $q$. Other terms rely on error bounds in the metric. We first take the null decomposition of $g$. Since $\overline{F}$ is supported on the exterior, we do not need to worry about singular behavior at the origin.

We have the uniform bound
\begin{equation}
|\overline{F}^{\sigma\gamma}\partial_\gamma g_{\alpha\sigma}| \lesssim \frac{q\epsilon}{\tp[3-\iota]\tm}.
\end{equation}
as well as the nicer bound
\begin{equation}
\left|\Ls^\alpha \overline{F}^{\sigma\gamma}\partial_\gamma g_{\alpha\sigma}\right| \lesssim \frac{q\epsilon}{\tp[3+\gamma'-\iota]\tm[1-\gamma']}
\end{equation}


These can be regarded as error terms. In particular, these scale with $q\epsilon$. Straightforward computation gives us that the current norm of these quantities is bounded by a constant times $q\epsilon$ as long as the growth constant $\delta$ of the weight is less than $\frac12$. Additionally, this estimate holds for Lie derivatives as long as components of $\Lie{Z^I}F$ are bounded by a constant times $q\tp[-2]$. For the first term, $g^{\beta\gamma}\partial_\gamma\overline{F}_{\alpha\beta}$, we will need to be more careful. We first take the null decomposition in $\gamma$ and look at the non-error terms. First, in the cases
\[
g^{\beta\Ls}\Ls(F_{\alpha\beta}), \quad g^{\beta\uLs}\uLs(F_{\alpha\beta}),
\]
we can commute our null vector fields through the derivative up to error terms decaying like $\epsilon\tp[-2+\iota]$, which when combined with the decay rate $q\tp[-2]$ of $F$ is easily absorbed into our current norm. First, we look at $\gamma = \Ls$. In this case, only $\beta = \uLs$ fails to have nice decay rates in our null decomposition. This contributes
\[
-\frac{q\overline{\chi}}{2\pi r^{*3}}
\]
to our $J_\Ls$ component. If $\gamma = \uLs$, we look at the case $\beta = \Ls$, in which case we have a non-error term like 
\[
-\frac{q\overline\chi}{2\pi r^{*3}} - \frac{q\overline\chi'}{2\pi r^{*2}}
\]
 in the $J_\uLs$ component.

 Likewise, for
\[
g^{\beta\Bs{j}}\Bs{j}(F_{\alpha\beta}),
\]
if $\beta \neq \Bs{j}$ when we take the null decomposition, we have decay like $\tp[-4+\iota]$, which suffices. We can treat this as $\Bs{j}^\beta \Bs{j}(F_{\alpha\beta})$ plus an error term with the same nice decay rate $q\tp[-4+\iota]$.
If $\beta = B_j$, we use the identity 
\[
B_i(B_i^\alpha) = \frac12 \partial_r(r^*)\frac{r}{r^{*2}}(\uLs-\Ls) + \frac{c_{ii}^j}{r^*}B_j.
\]
This contributes 
\[
\frac{q\overline\chi}{2\pi r^{*3}} + q\epsilon O(\tp[-4+\iota])
\]
to the $J_\uLs$ component and
\[
\frac{q\overline\chi}{2\pi r^{*3}}+ q\epsilon O(\tp[-4+\iota])
\]
to the $J_\Ls$ component. As usual the error terms do not present a problem. As for the non-error terms, we can divide 
\begin{equation}
\nabla^\beta \overline{F}_{\alpha\beta} = \overline{J}^1_\alpha + \overline{J}^2_\alpha,
\end{equation}
where $\overline{J}^1$ consists of the terms appearing in the Minkowski case, in particular the $J_\uLs$ term which is supported only when $\overline\chi' \neq 0$, and $J_2$, the set of other error terms. In each case, we can bound the current norms easily. We have in particular
\begin{equation}
\label{JNorm}
\lnorm \overline{J} \rnorm_{L^2[w]} \lesssim q.
\end{equation}

We now need to take an estimate on the current associated to Lie derivatives of $F$. We take, for any antisymmetric $(2,0)$-tensor $T$,
\begin{align}
[\nabla_\alpha, \Lie{Z}]T^{\alpha\beta} &= Z^\gamma[\nabla_\alpha, \nabla_\gamma] T^{\alpha\beta} - (\nabla_\alpha\nabla_\gamma Z^\alpha) T^{\gamma\beta} -(\nabla_\alpha\nabla_\gamma Z^\beta)T^{\alpha\gamma}, \nonumber\\
&= Z^\gamma R^\alpha_{\rho\alpha\gamma} T^{\rho\beta} + Z^\gamma R^\beta_{\rho\alpha\gamma}T^{\alpha\rho} - (\nabla_\gamma\nabla_\alpha Z^\alpha)T^{\gamma\beta} - R^\alpha_{\rho\alpha\gamma}Z^\rho T^{\gamma\beta} - \frac12 R^\beta_{\rho\alpha\gamma}Z^\rho T^{\alpha\gamma}, \\
&= -\nabla_\gamma(\nabla\cdot Z)T^{\gamma\beta}. \nonumber
\end{align}
Here in the last line we have used the symmetry of the Ricci curvature as well as the first Bianchi identity (combined with antisymmetry of $T$). 

Iterating this gives us
\begin{equation}
\label{FComms}
[\nabla_\alpha, \Lie{Z}^I]F^{\dagger\alpha\beta} = \sum_{\{Z^{I_1},Z_1,Z^{I_2}\} = Z^I}-\Lie{Z}^{I_1}\left(\nabla_\beta(\nabla\cdot Z_1)(\Lie{Z}^{I_2}(F^{\dagger}))^{\alpha\beta}\right).
\end{equation}
Here, $F^\dagger$ corresponds to $F$ with indices raised with respect to $g$ (before taking the Lie derivative). Since $\nabla\cdot Z_1$ is small, this can be regarded as a series of error terms. One immediate consequence of this is that we will have to bound the nice part of our current, $\overline{J}$ in the exterior by our metric energy norms. We write $F^{\dagger\alpha\beta} = g^{\alpha\gamma}g^{\beta\delta}F_{\delta\beta}$, and switch indices, to get
\begin{equation}
\label{CurrentComm}
\nabla_\beta\left(\Lie{Z}(g^{\alpha\gamma}g^{\beta\delta}F_{\gamma\delta})\right) = \Lie{Z}(\nabla^\gamma F_\gamma^\beta) + \nabla_\gamma(\nabla\cdot Z)F^{\dagger\gamma\beta}.
\end{equation}
Our goal is to bound the highest-order current norm $\lnorm J(\Lie{Z}^I\overline{F})\rnorm_{L^2[w]}$ by the energy. We do this inductively, first assuming all current norms
\[
\lnorm J(\Lie{Z}^K\overline{F})\rnorm_{L^2[w]}
\] are bounded for $|K| \leq |I| - 1$. We can expand
\begin{equation}
\nabla_\beta\left(\Lie{Z}^I(g^{\alpha\gamma}g^{\beta\delta}\overline{F}_{\gamma\delta})\right) = \Lie{Z}^I(g^{\alpha\gamma}\overline{J}_\gamma) + \sum_{\{Z^{I_1},Z_1,Z^{I_2}\} = Z^I}-\Lie{Z}^{I_1}\left(\nabla_\beta(\nabla\cdot Z_1)(\Lie{Z}^{I_2}(\overline{F}^{\dagger}))^{\alpha\beta}\right).
\end{equation}
We have three types of terms to worry about. First, we consider the first term on the right hand side, containint $\overline{J}$. We have the estimate
\begin{equation}
\left|\Lie{Z}\left(\overline{F}^{\sigma\gamma}\partial_\gamma g_{\alpha\sigma}\right)\right| \lesssim q\tp[-2]|\partial(\Lie{Z}(g)| + q\tp[-4+\iota]|\Lie{Z}g|,
\end{equation}
from which we see that the part of the current norm coming from this term is bounded by $\epsilon^2$, by taking our energy norms on $g$, subtracting off the $|\partial h_0|$ term, and our $L^\infty$ norms on $F$. More precisely:
\begin{equation}
\int_0^T\intsig{t}\tp[2s-3+2\iota]|\partial h_1|^2 w \lesssim E[g],
\end{equation}
with more decay coming from $h_0$ at the cost of having to integrating directly. the case with $g$ follows similarly, where we can integrate the well-behaved terms directly, and bound our error terms by the energy. We now look at other terms. 

==> ChJuly/Comparison.tex <==
This work can be seen as a expansion on results found by Lindblad and Sterbenz in \cite{LS}, who establish analogous estimates in Minkowski space. It is also worth mentioning results by \cite{BMS} in which they establish similar results for Minkowski space in a way that can more readily be generalized into a gauge-free geometric setting, and which could potentially provide better understanding of the precise asymptotic behavior in a relativistic metric. Further analysis by Shiwu Yang in \cite{Y152} and \cite{Y151} has expanded on these results, showing stability even when the electromagnetic field $F$ has large initial data. This approach uses the $r$-weighted energy decay method of \cite{DR} instead of the Morawetz estimate. This energy method was generalized to a broader class of metrics in \cite{M16}, and in \cite{S13}. Additionally, decay results for the massive Maxwell-Klein-Gordon system were found in \cite{KWY}, though due to the ``true" Klein-Gordon behavior of this system, results will be more difficult to generalize to a relativistic setting.

==> ChJuly/EMTensorBoundsDeleted.tex <==
\subsection{The Bounds on the Energy-Momentum Tensor}

We now show the desired bounds on the energy-momentum tensor. In all cases we naturally split $Q = Q^1+Q^2+Q^3+Q^4$, where
\begin{alignat*}{4}
Q^1_{\alpha\beta} &= \mathfrak{R}(D_\alpha\phi\overline{D_\beta\phi}),\qquad & Q^2_{\alpha\beta} &= \mathfrak{R}(g_{\alpha\beta}g^{\gamma\delta}D_\gamma\phi\overline{D_\delta\phi}),\\
Q^3_{\alpha\beta} &= F_{\alpha\gamma}F_\beta^{\,\,\,\gamma}, \qquad & Q^4_{\alpha\beta} &= g_{\alpha\beta}g^{\gamma\gamma'}g^{\delta\delta'}F_{\gamma\delta}F_{\gamma'\delta'}.
\end{alignat*}
Lie derivatives on each term behave differently. We first have the identities
\begin{subequations}
\begin{align}
(\Lie{X}^I Q^1)_{\alpha\beta} &= \sum_{|I_1|+|I_2|\leq |I|}\mathfrak{R}((\LieC{X}^{I_1}D\phi)_\alpha\overline{(\LieC{X}^{I_2}D\phi)_\beta}),\\
(\Lie{X}^I Q^2)_{\alpha\beta} &= \slk(\Lie{X}^{I_1}g)_{\alpha\beta}(\Lie{X}^{I_2}g^\dagger)^{\gamma\delta}\mathfrak{R}((\LieC{X}^{I_3}D\phi)_\gamma\overline{(\LieC{X}^{I_4}D\phi)_\delta})\\
(\Lie{X}^I Q^3)_{\alpha\beta} &= \slk(\Lie{X}^{I_1}g^\dagger)^{\gamma\gamma'}(\Lie{X}^{I_2}F)_{\alpha\gamma}(\Lie{X}^{I_2}F)_{\beta\gamma'}\\
(\Lie{X}^I Q^4)_{\alpha\beta} &= \slk(\Lie{X}^{I_1}g)_{\alpha\beta}(\Lie{X}^{I_2}g^\dagger)^{\gamma\gamma'}(\Lie{X}^{I_3}g^\dagger)^{\delta\delta'}(\Lie{X}^{I_4}F)_{\gamma\delta}(\Lie{X}^{I_5}F)_{\gamma'\delta'}
\end{align}
\end{subequations}


We show here the $L^1$ estimate for the good components, as the general $L^1$ estimate is quite a bit simpler.

 First, equation \eqref{L2SEM}:
\begin{Proposition}
Given the bounds of Theorem \ref{Main} as well as the energy estimates \eqref{EnergyPhi} and \eqref{EnergyF}, we have the estimate
\[
\sum_{|I| \leq k}\lnorm|\Lie{X}^IQ|_{\mcU\mcU}(t, \cdot)\langle(r^*-t)_+\rangle^{1/2+\gamma}\rnorm_{L^2(x)} \lesssim \epsilon^2(1+t)^{-1},
\]
where we say
\[
|T|_{\mathcal{X}\mathcal{Y}} = \sup_{X \in \mathcal{X}, Y \in \mathcal{Y}} |T_{XY}|.
\]
\end{Proposition}
\begin{proof}
We first expand $\Lie{X}^I Q(U,V)$, for $U,V \in \mathcal{U}$. We fortunately don't need to take our null frame into account, which makes our calculations easier. We first note the following three estimates, recalling the definition $\OLie{X}(g) = \Lie{X}(g)- c_Xg$ for the standard metric, and $\OLie{X}(g^\dagger) = \Lie{X}(g^\dagger) + c_Xg^\dagger$ for the inverse metric:
\begin{align*}
\sum_{|I| \leq k-6}|\LieC{X}^ID\phi|_{\mcU} + |\Lie{X}^IF|_{\mcU\mcU}) &\lesssim \epsilon\tp[-1]\tm[-1], \\
\sum_{|I| \leq k}|\Lie{X}^I\overline{F}|_{\mcU\mcU}&\lesssim \epsilon\tp[-2], \\
\sum_{|I| \leq k-6}|\Lie{X}^Ig|_{\mcU\mcU} & \lesssim 1.
\end{align*}
The estimates on derivatives of $F$ follow directly from \eqref{ChargeLInfty} and \eqref{est:FTLinfty}. The estimate on $F$ comes from the identity
\[
|(\LieC{X}^ID\phi)_U| \lesssim |D_UD_X^I\phi| + \sum_{|I_1|+|I_2|+1 \leq |I|}|(\Lie{X}^{I_1}F)(X_1, U)D_X^{I_2}\phi|,
\]
combined with an application of \eqref{ChargeLInfty} and \eqref{est:FTLinfty} on the terms containing $F$ and \eqref{est:LinftyDPhi} on the terms containing $\phi$.

In order to prove estimates on $\Lie{X}^IQ$, we consider several steps. First, we decompose $F = \widetilde{F} + \overline{F}$, and $g = m^0+H$, $g^\dagger = m_0+h$, and expand $\Lie{X}^I Q$.  Then, we get three types of terms. First, we have terms containing terms like $|\overline{F}|^2$ where $k-6$ or fewer derivatives fall on any terms containing $g$. In these cases, we can bound the integral
\begin{align*}
\sum_{|I| + |J| \leq k}\lnorm|\Lie{X}^I\overline{F}||\Lie{X}^J\overline{F}|\langle(r^*-t)_+\rangle^{1/2+\gamma}\rnorm_{L^2(x)} &\lesssim \epsilon^2 \lnorm \langle t+r \rangle^{-4 + 1/2 +\gamma} \rnorm_{L^2(x)} \\
 &\lesssim \epsilon^2(1+t)^{-1} \lnorm \langle t+r \rangle^{-5/2 +\gamma} \rnorm_{L^2(x)} 
\end{align*}.
We note that, since $-5/2 + \gamma < -3/2$, the right hand side is bounded in $L^2(x)$. Next, we look at terms containing Lie derivatives of terms like $|D\phi|^2$ or $|F||\widetilde{F}|$, and where $k-6$ or fewer derivatives fall on any terms containing $g$. For the terms like $|F||\widetilde{F}|$. without loss of generality, we assume we can use $L^\infty$ estimates on $|F|$ and $L^2$ estimates on $|\widetilde{F}|$. In these cases, we can bound
\[
\sum_{\substack{|I| + |J| \leq k \\ |I| \leq k-6}}\lnorm|\Lie{X}^IF||\Lie{X}^J\widetilde{F}|\langle(r^*-t)_+\rangle^{1/2+\gamma}\rnorm_{L^2(x)} \lesssim \epsilon (1+t)^{-1}\sum_{|J|\leq k}\lnorm|\Lie{X}^J\widetilde{F}| \langle{r^*-t}\rangle^{-1/2+\gamma}\rnorm_{L^2(x)}
\]
Our result follows from the inequality $\gamma-1/2 < s$. We now consider the terms where most derivatives fall on the metric. We note that by decomposing using the modified Lie derivative $\widetilde{L}$ and bounding the terms containing $c_Xg$ similarly to the prior two cases, we can reduce this to terms containing $L^2$ norms of $\OLie{X}g$ and $\OLie{X}(g^\dagger)$. We treat each of these the same way. In particular, we note that these are paired with Lie derivatives of $|D_X\phi|^2$ or $|F|^2$, both of which are bounded in $L^\infty$ by $\epsilon\tp[-2]\tm[-2]$. We therefore have the estimate
\begin{align*}
\sum_{\substack{|I| + |J| + |K| \leq k \\ |I| + |J| \leq k-6}}&\lnorm(|\Lie{X}^IF| + |D_X^I\phi|)(|\Lie{X}^JF| + |D_X^J\phi|)|\OLie{X}^K g|\langle(r^*-t)_+\rangle^{1/2+\gamma}\rnorm_{L^2(x)} \lesssim \\
&\lesssim \sum_{|K|\leq k}\epsilon^2(1+t)^{-3/2}\lnorm\tm[-1]|\OLie{X}^K g|\rnorm
\end{align*}

Now we prove the $L^1$ estimates on derivatives of $Q$.
\end{proof}


\begin{Proposition} With assumptions and notation as in Theorem \ref{Main}, 
we have the bounds on the energy-momentum tensor
\begin{subequations}
\begin{align}
\label{L2SEM}
\sum_{|I| \leq k}\lnorm|\Lie{X}^IQ(t, \cdot)|\langle(r^*-t)_+\rangle^{1/2+\gamma}\rnorm_{L^2(x)} &\lesssim \epsilon^2\langle t \rangle^{-1}, \\
\label{L1SEM}
\sum_{|I| \leq k}\lnorm|\Lie{X}^IQ(t, \cdot)|\rnorm_{L^1(x)} &\lesssim\epsilon^2, \\
\sum_{|I| \leq k}\lnorm|\Lie{X}^IQ(t, \cdot)|_{\mcU\mcT}\rnorm_{L^1(x)} &\lesssim\epsilon^2(1+t)^{-s},
\end{align}
\end{subequations}
where $Q$ is defined as in \eqref{FullEMTensor}. We additionally have the $L^\infty$ estimates on lower-order derivatives
\begin{subequations}
\begin{align}
\sum_{|I| \leq k-6}|\Lie{X}^IQ(t, \cdot)|_{\mcU \mcU} &\lesssim \epsilon^2\tp[-2]\tm[-2] \\
\sum_{|I| \leq k-6}|\Lie{X}^IQ(t, \cdot)|_{\mcU\mcT} &\lesssim \epsilon^2\tp[-2-s]\tm[-2+s] \\
\sum_{|I| \leq k-6}|\Lie{X}^IQ(t, \cdot)|_{\mcL\mcT} &\lesssim \epsilon^2\tp[-5/2-2s]\tm[-3/2+2s]
\end{align}
\end{subequations}

\end{Proposition}


==> ChJuly/IntroHansSuggestion.tex <==
In this paper we prove stability and decay rates for solutions of  the massless Einstein-Charge Scalar Field system, also called the massless Einstein-Maxwell-Klein-Gordon system, on an asymptotically flat metric close to Minkowski space.

First, given a background spacetime $(\mathcal{M}, g)$ and a real one-form $A$, one can define the complex covariant derivative
\begin{equation}
D_\alpha = \nabla_\alpha + iA_\alpha,
\end{equation}
where $\nabla$ is the Levi-Civita connection on $g$.
Then, for the two-form $F = dA$ and a complex scalar function $\phi$, the massless Charge-Scalar Field system is defined as follows:
\begin{subequations}
\label{MKG}
\begin{align}
D^\alpha D_\alpha \phi &= 0, \\
\label{currentvector}
\nabla^\beta F_{\alpha\beta} &= \mathfrak{I}\left(\phi\overline{D_\alpha\phi}\right), \\
\nabla^\beta( {^*}F)_{\alpha\beta} &= 0.
\end{align}
\end{subequations}
Here and in what follows, $\mathfrak{R}, \mathfrak{I}$ denote the real and imaginary parts of a quantity respectively.

Given this system along with suitable initial conditions for $F$ and $\phi$, one has some freedom in the choice of the potential $A$ which it is not necessary to resolve. These quantities are tied together by the commutator relation
\begin{equation}
\label{commrelation}
[D_\alpha, D_\beta]\phi = iF_{\alpha\beta}\phi.
\end{equation}

The right hand side of \eqref{currentvector} is the current vector, $J_\alpha$, and was selected as such in order to make the combined energy-momentum tensor,
\begin{equation}
\label{FullEMTensor}
Q_{\alpha\beta}[\phi, F] = \mathfrak{R}\left(D_\alpha\phi\overline{D_\beta\phi} - \frac12g_{\alpha\beta}D_\gamma\phi\overline{D^\gamma\phi}\right) + F_{\alpha\gamma}F_\beta^\gamma - \frac14g_{\alpha\beta}F_{\gamma\delta}F^{\gamma\delta},
\end{equation}
divergence free. We separate this tensor into its scalar and field quantities, respectively
\begin{subequations}
\begin{align}
Q_{\alpha\beta}[\phi] &= \mathfrak{R}\left(D_\alpha\phi\overline{D_\beta\phi} - \frac12 g_{\alpha\beta}D_\gamma\phi\overline{D^\gamma\phi}\right), \\
Q_{\alpha\beta}[F] &= F_{\alpha\gamma}F_\beta^\gamma - \frac14g_{\alpha\beta}F_{\gamma\delta}F^{\gamma\delta}.
\end{align}
\end{subequations}
These satisfy the identities
\begin{equation}
\nabla^\beta Q_{\alpha\beta}[\phi] = F_{\alpha\gamma}J^\gamma, \qquad \nabla^\beta Q_{\alpha\beta}[F] =  -F_{\alpha\gamma}J^\gamma,
\end{equation}
which follow from the commutator identity \eqref{commrelation} along with the identity
\begin{equation}
\nabla_\alpha(\phi\overline{\psi}) = D_\alpha\phi\overline\psi + \phi\overline{D_\alpha\psi}
\end{equation}
in the scalar term, and antisymmetry along with the identity
\begin{equation}
\nabla_\alpha F_{\beta\gamma} + \nabla_\beta F_{\gamma\alpha} + \nabla_\gamma F_{\alpha\beta} = 0
\end{equation}
in the electromagnetic term.

We consider spacetimes $(\mathcal{M}, g)$ close to Minkowski, in the sense that they satisfy certain $L^2$ and $L^\infty$ estimates consistent with small-data solutions to Einstein's Vacuum Equations in harmonic gauge. We in particular assume certain energy norms consistent with the stability result \cite{LR}, combined with nicer $L^\infty$ estimates on certain components of the metric shown in \cite{L15}, for a metric with small initial data. We note that we require better decay on the initial data than the previous two works, in the sense that they require the mass-free part of the perturbation to decay only like $r^{-1-\alpha}$ at infinity (for any $\alpha > 0$), while we require it to decay better than $r^{-3/2-\alpha}$.

There is a natural way to frame these $L^\infty$ results, which comes from the mass corresponding to the metric. We assume the metric is of the form
\begin{equation}
\label{Metric}
g_{\alpha\beta} = m _{\alpha\beta} + \left(\frac{M\chi}{1+r}\right)\delta_{\alpha\beta} + h_{\alpha\beta},
\end{equation}
where $M$ is a small constant corresponding to the ADM mass, $h$ is a small $(0,2)$-tensor, and $\chi$ is a smooth cutoff function equal to 1 for $r > 3t/4$ and 0 for $r < t/2$, such that $\partial\chi$ decays like $t^{-1}$.

This metric corresponds to small-data solutions of the Einstein Vacuum Equations, as well as a range of coupled Einstein-field systems. In particular, it is our hope that the stability results here can be used as a priori estimates which can prove the stability of the Einstein-massless Charge Scalar Field system, which in harmonic coordinates can be written as the system \eqref{MKG} in a metric satisfying the system
\begin{equation}
\Box_g(g_{\mu\nu}) = P_{\mu\nu}(g)(\partial g, \partial g) +C(Q_{\mu\nu} - \frac12\text{tr}(Q)),
\end{equation}
where $Q$ is the quantity in equation \eqref{FullEMTensor}, and $P$ is quadratic in derivatives of $g$ with nice asymptotic properties in the null decomposition of $g$. This set of nice asymptotic properties is in particular known as the weak null condition.

We can think of small-data solutions of the MKG equations as solutions for the Einstein-Field Equations with small $C$, so that for at least a long time the system takes place on a metric which is mostly unaffected by solutions of the Charge-Scalar Field system. Global existence will ideally follow from estimates on $Q$ which follow from these results, from the fact that we have nicer energy and decay estimates for this tensor than for terms corresponding with terms on the right hand side coming from $g$.

We note that in the wave zone $t \approx r$ and in the exterior, our metric behaves similarly to Schwarzschild, which requires some additional geometric consideration even for large $r$. Here, we draw geometric inspiration from analysis of solutions to wave equations in Schwarzschild carried out by Blue and Sterbenz in \cite{BS06}, where they take the conformal Morawetz estimate with $r, \partial_r$ replaced by the tortoise coordinate and derivative $r^*$ and $\drs$. We can consider the approximate optical functions $\us = t + r^*$, $\uls = t - r^*$.

In our case, we cannot hope to recover the full conformal Morawetz estimate using only the geometric structure of these approximate optical functions, due to insufficient decay in perturbations of the metric. However, we can establish a fractional Morawetz estimate, analogous to that in \cite{LS}, for certain fractional weights $\us[2s], \uls[2s]$ which depend on the initial spatial decay of the metric. We show the base estimate, along with a discussion on why the fractional estimate and curved fields are necessary, in section \ref{ModelMorawetz}.

Our primary tool here is a null decomposition and a set of vector fields which are defined only in terms of the parameter $M$ which behave nicely with respect to the metric $\mt = m + M\chi/(1+r)\delta$ This set of Lorentz fields was used in  \cite{L15} to establish nicer asymptotic behavior for certain components of the metric. The null decomposition we use is a natural extension of these fields, and allows us to establish nicer estimates on certain derivatives of $\phi$ and components of $F$ than the corresponding null fields in Minkowski would.

In order to define these fields, we define the adapted tortoise coordinate,
\[
r^* = r + M\chi\ln(1+r),
\]
such that $\chi = \tilde{\chi}(r/t)\tilde{\chi}(r)$, where $\tilde{\chi}$ is a smooth increasing function satisfying
\[
\tilde{\chi}(y) = \begin{cases} 1 & y \geq 3/4 \\ 0 & y \leq 1/2\end{cases}.
\]
For $t > 1$, $r^* = r$ in the far interior $r < t/2$ and $r^* = r+M\ln(1+r)$ in the extended exterior region, $r > 3t/4$. We can use this quantity to define the modified coordinates
\begin{equation}
\us = t - r^*, \qquad \uls = t + r^*, \qquad t^* = t, \qquad \xsi{i} = \omega^ir^*.
\end{equation}
We note that $\us$ and $\uls$ are not quite optical functions of the metric, in the sense that $g^{\alpha\beta}\partial_\alpha \us\partial_\beta\us \neq 0$. However, $\us$ can be seen as a sufficient approximation (more so than $u = t-r$, one optical function for the Minkowski metric). Additionally, we can define the optical weights
\begin{equation}
\label{taupm}
\tp[2] = (1+\uls[2]) \qquad \tm[2] = (1+\us[2]) \qquad \tz = \tm/\tp.
\end{equation}

Given $\partial_r = \omega^i\partial_i$ and $\opar_i = \partial_i - \omega_i\partial_r$, we can define
\begin{equation}
\drs = \frac{1}{\partial_r(r^*)}\partial_r, \qquad \dts = \dxsi{0} = \partial_t - \partial_t(r^*)\drs, \qquad \dxsi{i} = \omega_i \drs + \frac{r}{r^*}\opar_i.
\end{equation}
We write
\[
\ops{i} = \frac{r}{r^*}\opar_i,
\]
a quantity which will often come up naturally later when calculating commutators.

This choice of fields lends itself to a natural null frame,
\begin{equation}
\Ls = \dts + \drs, \qquad \uLs = \dts - \drs, \qquad S_i^* = \frac{r}{r^*}S_i,
\end{equation}
where $S_i = \{S_1, S_2\}$ are piecewise defined fields forming an orthonormal frame tangent to the sphere (in the Minkowski metric). We note that our use of $S^*_i$ is not strictly necessary, as they are of course proportional to $S_i$ with a scalar factor close to 1; however, their use elucidates several cancellations which are necessary in handling Lie derivatives of the EM field, and which are not at all obvious using $S_i$ alone. We use the shorthand
\begin{equation}
\mcL = \{\Ls\}, \qquad \mcT = \{\Ls, S_1^*, S_2^*\}, \qquad \mcU = \{\Ls, \uLs, S_1^*, S_2^*\}.
\end{equation}

This correspondence between our  frames and fields have two advantages: First, they correspond well with estimates on the metric, for which one has the nice component estimate
\[|g_{\mcL\mcT}| \lesssim \frac{\epsilon\tm[\gamma']}{\tp[1+\gamma'-\delta']},
\]
where $\gamma'$ and $\iota$ are defined as in \eqref{MetLI} and \eqref{MetL2}. This makes it possible to achieve nicer estimates on the deformation tensor $\Lie{Z}g$ without having to take into account the full geometric structure. This first comes into play in our energy estimates, where we must bound terms roughly behaving like
\[
\int_0^T\intsig{t}|(\Lie{\okos}g)(\Ls,\Ls)||D_\uLs\phi|^2w \, dx \, dt,
\]
where
\[\okos =\frac12(1+\uls[2s])\Ls + \frac12(1+\abus[2s])\uLs.\]

In order for this to be bounded by our energy, we need $\Lie{\okos}g(\Ls, \Ls)$ to be bounded roughly by $\epsilon\tm[2s]\tp[-1-\alpha]$, for some $\alpha > 0$. This estimate is in particular not possible when we replace $\Ls$ by its Minkowski analogue $\partial_t+\partial_r$ due to the behavior of the part of the metric like $M\chi/(1+r) \delta$. In the latter case, we would get decay like $\tp[2s-2]$ which would lead to polynomial growth in the energy even in the border case $s=1/2$. It might be possible to mitigate this by subtracting off quantities close to the light cone, but this would be unintuitive without the geometric understanding of our modified fields.

Additionally, this null frame commutes well with the modified Lorentz fields used in \cite{L15}, which again seem to be necessary in order to get the desired decay of metric terms. This follows from the fact that we would expect Lie derivatives of components of $F$ to satisfy similar estimates to Lie derivatives of $F$. In the null frame in Minkowski, the best decay we would be able to expect for components like $|\Lie{Z}^{I}F_{\Ls S_j}|$ would be $\tp[-2]\tm[1/2-s]$, as opposed to the analogous term in \cite{LS}, for which we would get the improved decay rate $\tp[-3/2-s]$.

 We contrast this to \cite{LR}, which required less delicate peeling estimates, and consequently for which the standard null frame for Minkowski space sufficed.

We define the adapted null decomposition of $F$ as follows:
\begin{subequations}
\begin{alignat}{4}
\alpha_i &= F_{\Ls\Bs{i}} & \qquad\ual_i &= F_{\uLs \Bs{i}} \\
\rho &= \frac12F_{\uLs\Ls} & \sigma &= \frac12F_{\Bs{1}\Bs{2}}
\end{alignat}
\end{subequations}

Since the tangential terms are not uniquely defined, the following terms often show up in our calculations.
\[
|D_{\Bs{}}\phi|^2 = |D_{\Bs{1}}\phi|^2 + |D_{\Bs{2}}\phi|^2 \qquad |\al|^2 = |\al_1|^2 + |\al_2|^2 \qquad |\ual|^2 = |\ual_1|^2+|\ual_2|^2.
\]

We additionally define the electromagnetic decomposition
\begin{equation}
E_i = F_{0i}, B_i = (*F)_{0i},
\end{equation}
where $*F$ is the Hodge dual of $F$.
We can break $E$ up into its divergence-free and curl-free components, $E_{df}$ and $E_{cf}$ respectively.

Before stating our result, we define the norms governing our initial conditions. For a $(0,k)$-tensor $T$, we define:

\begin{equation}
\left\lVert T\right\rVert^2_{H^{k, s_0}(\mathbb{R}^3)} = \sum_{|I| \leq k} \sum_{\alpha_k \in (0,3)}\int_{\mathbb{R}^3} (1+r^2)^{s_0+|I|}|\underline\nabla^I T(\dxsi{\alpha_1}, ...\dxsi{\alpha_k})|^2 \, dx,
\end{equation}
where $I$ is a multiindex. Here, $\underline\nabla$ and $\underline{D}$ are the covariant derivatives restricted to time slices.

Likewise, for a complex scalar field, we have the corresponding quantity
\begin{equation}
\left\lVert \phi\right\rVert^2_{H^{k, s_0}(\mathbb{R}^3)} = \sum_{|I| \leq k} \int_{\mathbb{R}^3} (1+r^2)^{s_0+ |I|}|\underline{D}^I \phi|^2 \, dx.
\end{equation}

\begin{Theorem}
\label{Main}
Take constants $s_0, \gamma', \delta$ such that $\frac12 < s_0-\delta < \gamma' < 1 < s_0$, and $\iota$ such that the difference between any two of the previous quantities is at least $4\iota$. Additionally, take an integer $k_0 \geq 11$.

There exists a constant $\epsilon_0 > 0$, with $\epsilon_0 \ll \iota$, such that if the metric satisfies \eqref{MetLI} and \eqref{MetL2} for $\epsilon < \epsilon_0$, and if we take initial conditions $E_0, B_0, \phi_0, \dot{\phi}_0$ for $F$ and $\phi$ satisfying

\begin{equation}
\left\lVert E_{0df} \right\rVert_{H^{k_0, s_0}(\mathbb{R}^3)} + \left\lVert B_0 \right\rVert_{H^{k_0, s_0}(\mathbb{R}^3)}+ \left\lVert D\phi_0 \right\rVert_{H^{k_0, s_0}(\mathbb{R}^3)} + \left\lVert\dot\phi_0 \right\rVert_{H^{k_0, s_0}(\mathbb{R}^3)} < \epsilon
\end{equation}
at time $t = 0$, then solutions to \eqref{MKG} exist for all time and satisfy the bounds
\begin{subequations}
\begin{align}
|\alpha| + \left|\frac{1}{r^*}D_{\Ls}(r^*\phi)\right|\chi_{r^* > t/2+1/2} + |D_{\Ls}\phi|\chi_{r^* < t/2 + 1/2} &\lesssim \epsilon\tp[-s-3/2], \\
|\ual| + |D_{\uLs}\phi| &\lesssim \epsilon\tp[-1]\tm[-1/2-s], \\
|\sigma|  &\lesssim \epsilon\tp[-1-s]\tm[-1/2],\\
|\slashed{D}\phi| &\lesssim \epsilon\tp[-2]\tm[1/2-s],\\
|\rho| &\lesssim \epsilon\left(\tp[-1-s]\tm[-1/2]\chi_{r^* < t} + \tp[-2]\chi_{r^* \geq t}\right), \\
|\phi| &\lesssim \epsilon\tp[-1]\tm[1/2-s],
\end{align}
\end{subequations}
for $s = s_0 - \delta$, and $\tau_\pm$ as defined in equation \eqref{taupm}.

Moreover we have similar estimates for Lie Derivatives with respect to vector fields applied to $\phi$ and $F$. , see Proposition ...

\end{Theorem}
An integral part of the proof is to prove higher order energy bounds which are also interesting:
\begin{Proposition} With assumptions as in Theorem \ref{Main}, for all $t$, we have the energy bounds on derivatives of $\phi$ as follows:
\begin{equation}
\mathcal{E}_k[\phi](t) = \sum_{|I|\leq k}E_0[D_X^I\phi](t) \leq C\epsilon,
\end{equation}
where
\[
E_0[\psi](T) = \sup_{0 \leq t \leq T}\intsig{t}\left(\tp[2s]\left(\left|\frac{D_\Ls(r^*\psi)}{r^*}\right|^2 + |\slashed{D}\psi|^2 + \left|\frac{\psi}{r^*}\right|^2\right) + \tm[2s]|D_\uLs\psi|^2\right) w \, dx
\]
Here, $I$ is a multiindex of the Lorentz fields $X \in \mathbb{L}$, as defined in \eqref{LorentzFields}, and $w$ and $w'$ are weight quantities defined in \eqref{WeightDefs}

Moreover we have similar estimates for the electromagnetic field.....

Moreover, there is a spacetime part see Proposition.... 
\end{Proposition}
When coupling this to Einstein's equations we need estimates for the energy momentum tensor:
\begin{Corollary} With assumptions as in Theorem \ref{Main} we have the follwing estimates for
the energy-momentum tensor
\begin{subequations}
\begin{align}
\label{L2SEM}
\sum_{|I| \leq k}\lnorm\Lie{X}^IQ(\mcU, \mcU)(t, \cdot) w\rnorm_{L^2(x)} &\lesssim \epsilon\lvert t \rvert^{-1} \\
\label{L1SEM}
\sum_{|I| \leq k}\lnorm\Lie{X}^IQ(\mcU, \mcU)(t, \cdot)\rnorm_{L^1(x)} &\lesssim\epsilon^2,
\end{align}
\end{subequations}
where $Q$ is defined as in \eqref{FullEMTensor}.

Moreover we have the following decay estimates for components of $Q$:..
\begin{align}
|Q|&\leq \epsilon t^{-1}\\
|Q_{TS}&\leq...\\
\end{align} 
where $S,T$ are tangential. 

We also have similar estimates for components of ${\mathcal L}_X^I Q$ see Proposition ...

\end{Corollary}

The proof of this theorem structurally follows the space-time energy approach of \cite{LS}, taking advantage of fractional Morawetz estimates used in that paper. The main conceptual difference is in the mass-corrected null frame and Lorenz fields. Additionally, there are significant error terms coming from the metric, which means that the required energy and commutator estimates are significantly more involved. Definitions and certain properties of these fields are outlined in section 2.

The last portion of section 2 includes several Morawetz estimates which provide motivation for the frameworks we use, including the fractional Morawetz estimate, the modified null frame, and the weight $w$. This estimate has at the end a discussion on certain issues adapting the full conformal Morawetz estimate to a general relativistic metric, and will hopefully cast light on our reasons for the fractional Morawetz estimate and the modified null frame and vector fields we use.

In sections 3 and 4, we first establish a fractional Morawetz estimate for the electromagnetic and scalar fields respectively. In the electromagnetic case, the proof is roughly straightforwardly adapted from \cite{LS}, in which we consider the fractional acceleration field
\[
\okos = \frac12\left((1+\uls[2s])\Ls + (1+\abus[2s])\uLs\right)
\]
for some constant $s \in (1/2, \gamma')$. The deformation tensor of this field satisfies certain positivity properties which were shown in \cite{LS}, with error terms coming from the metric which we bound straightforwardly. Additionally, we subtract off a charge quantity $\overline{F}$ and analyzing the remainder tensor $F-\overline{F}$, as analyzing $F$ on its own would result in field terms with insufficient decay in space.

For the scalar field, slightly more work is required, as the energy-momentum tensor is no longer trace-free. Therefore, we cannot rely on only the quasi-conformal killing structure of $\okos$. We instead take a conformal transformation of the metric and apply the energy estimate to solutions of the wave equation on this new metric, then augment the resulting estimate using a weighted Poincar\'e-type inequality, loosely adapted from a similar estimate in \cite{H}.

Sections 5 and 6 establish $L^\infty$ estimates on field quantities. These are conceptually straightforward weighted Klainerman-Sobolev estimates, with some additional care taken to account for the contribution of the charge. and issues establishing an energy norm along the light cone. Our estimates are Theorems \ref{LInftyF} and \ref{LinftyPhi}.

In sections 7 and 8 we bound commutator terms coming from taking the energy estimate on Lie and complex covariant derivatives of $F$ and $\phi$ respectively. This is achieved through a combination of the bilinear estimates used in \cite{LS} and a set of energies defined on the metric, which are bounded for a class of small-data solutions to the Einstein vacuum equations. In section 7.1 we also show that certain norms relating to initial data are equivalent or bounded by the initial data norms used in the main theorem.

Section 9 ties everything together: this will in particular establish that the right hand side of the earlier energy estimates can be easily bounded by the left hand side times a constant scaling with the size of the initial data. It follows that, for sufficiently small initial data, the energy is bounded. In particular, all parts of Theorem \ref{Main} follow directly from Theorem \ref{Bootstrap}.

Section 10 is an appendix which contains some weighted Poincare- and Sobolev-type estimates which are of use in our proof. 

==> ChJuly/L2phi__Chris_Kauffman_s_conflicted_copy_2021-07-22_.tex <==
We now establish a conformal energy estimate for a generic function $\phi$. Our approach in the exterior will be modeled by \cite{BS06}, as since no geodesics are trapped we do not need the time invariant estimate of \cite{DR}. Our approach largely follows that of Section \ref{ModelMorawetz}, with additional improvements on $\frac{\phi}{r}$. 

We recall the conformal Killing field
\[
K_0 = \frac12(\underline{u}^2(\partial_t+\partial_r) + u^2(\partial_t - \partial_r)).
\]
Applying the energy estimate will give a term like $t(\text{tr }Q[\bphi])$, (which vanished for $Q[\bG]$). In the Minkowski space one could use
\[
{^I}m = \tfrac{1}{r^2}m,
\]
in which $K_0$ is indeed Killing away from the spatial origin, and combine it with a similar estimate using the fundamental solution of the wave equation (cf. \cite{LS}). However, we will instead use a Hardy-type estimate which seems more robust under metric perturbations.

In any Lorentzian metric we have the commutator
\begin{equation}
\label{rBoxComm}
\Box_g^{\mathbb{C}}\phi = \Box\Big(\tfrac{1}{r^*}(r^*\phi)\Big) = \tfrac{1}{r^*}\Box_g^{\mathbb{C}}(r^*\phi) + 2\nabla^\alpha\Big(\tfrac{1}{r^*}\Big)D_\alpha(r^*\phi) + \Box_g\Big(\tfrac{1}{r^*}\Big)(r^*\phi)
\end{equation}

The singular behavior near the spatial origin is of concern, as in a general metric we can no longer consider $\frac{1}{r^*}$ as a solution of the wave equation for general metrics. We instead show take an estimate with a background metric $\mhat$ and deal with the remainder separately.

We recall the modified Minkowski metric $\mhat$, as defined in \ref{def:hatm}, and define
\begin{subequations}
\begin{equation}
\label{TSEnergyPhiD}
E_0[\phi](T) = \sup_{0 \leq t \leq T}\intsig{t}\left(\tp[2s]\left(\left|\tfrac{D_\Ls(r^*\phi)}{r^*}\right|^2 + |\slashed{D}\phi|^2 + \left|\tfrac{\phi}{r^*}\right|^2\right) + \tm[2s]|D_\uLs\phi|^2\right) w \, dx.
\end{equation}
It follows from Lemma \ref{HardyEstimate} that this is equivalent to
\begin{equation}
\label{TSEnergyPhiE}
\sup_{0 \leq t \leq T}\intsig{t}\left(\tp[2s]\left(\left|\tfrac{D_\Ls(r^*\phi)}{r^*}\right|^2 + |\slashed{D}\phi|^2\right) + \tm[2s]\left|\tfrac{D_\uLs(r^*\phi)}{r^*}\right|^2\right) w \, dx.
\end{equation}
\end{subequations}

Likewise, we have the interior spacetime energy
\begin{equation}
\label{STEnergyPhiD}
S_0[\phi](T) = \int_0^T \intsig{t}\left(\tp[2s]\left|\tfrac{D_\Ls(r^*\phi)}{r^*}\right|^2 + \tz[1+2\overline{\mu}]\left(\tp[2s]\left(|\slashed{D}\phi|^2 +\left|\tfrac{\phi}{r^*}\right|^2 \right) + \tm[2s]\left(|D_\uLs\phi|^2 \right)\right)\right) w' \, dx \, dt.
\end{equation}
and the light-cone energy
\begin{equation}
C_0[\phi](T) = \sup_{\us}\int_{C(\us)} T(\nabla \us,  \okos) w \, dC(\us),
\end{equation}
where $T$ is defined in equation \eqref{EMPhi}. $C_0$ is again no longer positive definite. For now we define the positive definite conical energy
\[
C_0^+[\phi](T) = \sup_{\us}\int_{C(\us)}\left(\left|\tp[2s]\frac{D_{\Ls}(r^*\phi)}{r^*}\right|^2 + \tm[2s]\sum_i\left|D_{\Bs{i}}\phi\right|^2 + \tp[2s]\tz[2]\left|\frac{\phi}{r^*}\right|^2\right)w \, dVC(\us).
\]
We will show later
\[
|C_0^+[\phi](T)| \lesssim C^{-1}(|C_0[\phi](T)| + \varepsilon_g |E_2[\phi](T)|).
\]
 We take the combined energy
\begin{equation}
\mathcal{E}_0[\phi](T) = E_0[\phi](T) + S_0[\phi](T) +  C_0[\phi](T)
\end{equation}
In general, we define
\begin{equation}
\mathcal{E}_k[\phi](T) = \sum_{\substack{|I| \leq k}} \mcE_0[D_X^I\phi](T).
\end{equation}
We can define the analogous quantities $E_k[\phi](T)$, $S_k[\phi](T)$, $C_k[\phi](T)$ similarly.

We recall the a priori assumption $\mathcal{E}_k[\phi](T) < C$, so in particular $\mathcal{E}_0[\phi](T)^m \leq \mathcal{E}_0[\phi](T)$ for $m \geq 1$.

We take the opportunity here to define the full energy
\begin{equation}
\mathcal{E}_k(T) = \mathcal{E}_k[\bphi] + \mathcal{E}_k[\bF^1] + |q[\bF]|^2,
\end{equation}
When there is no ambiguity we write $\mathcal{E}_k$.

We can now state the main theorem of this section.
\begin{Theorem}
\label{L2PhiMain}
For a given function $\phi$ with sufficient decay, we have
\begin{equation}
\mathcal{E}_0[\phi](T) \lesssim \mathcal{E}[\phi](0) + \left(|q|+\lnorm {\bF^1} \rnorm^{red}_{L^{\infty}[w]}\right)\mathcal{E}_0[\phi](T) + \lnorm \tp[s]\tm[1/2](\Box_g^{\mathbb{C}}\phi) w_{\delta}^{1/2}\rnorm_2^2,
\end{equation}
where we define the reduced weighted $L^\infty$ norm
\begin{equation}
\label{def:Fred}
\lnorm {\bF^1} \rnorm^{red}_{L^{\infty}[w]} = \sup_{[0,T]\times\mathbb{R}^3}\tp\tm[1/2+s]\ual[{\bF^1}]w^{1/2} + \tp[1+s]\tm[1/2](|\rho[{\bF^1}]| + |\sigma[{\bF^1}]|)w^{1/2} + \tp[3/2+s]|\al[{\bF^1}]|w^{1/2}.
\end{equation}
\end{Theorem}
In order to prove this, we will first show the estimate for the modified metric using \eqref{FirstEEPhi}, then handle the error terms using Lemma \ref{RemainderDivergence}.
\begin{Remark}
For the majority of this section we will raise and lower the metric with respect to ${\mhat}$. To reduce ambiguity we will use the notation 
\[
\nabla_{\mhat}^\alpha = \mhat^{\alpha\beta}\nabla_\alpha, D_{\mhat}^\alpha = \mhat^{\alpha\beta}D_\alpha.
\]
\end{Remark}

We note the following inequalities which will be used many times in the future.
\begin{subequations}
\label{STEnergy}
\begin{align}
\label{STEA}
\lnorm \tp[-1/2-\delta]\tm[s]|D\phi|w^{1/2} \rnorm_2^2 &\lesssim E_0[\phi](T) \\
\label{STEA2}
\lnorm \tp[s-1-\gamma'/2 + \delta/2]\tm[\gamma/2]|D\phi|w^{1/2} \rnorm_2^2 &\lesssim E_0[\phi](T) \\
\label{STEB}
\lnorm \tp[s-3/2-\delta]|\phi|w^{1/2} \rnorm_2^2 &\lesssim E_0[\phi](T) \\
\label{STEC}
\lnorm \tp[s-1/2-\delta]|\overline{D}\phi|w^{1/2} \rnorm_2^2 &\lesssim E_0[\phi](T) \\
\label{STED}
\lnorm \tp[2s-2+\delta]|\overline{D}\phi||D\phi|w\rnorm_1 &\lesssim E_0[\phi](T) \\
\label{STEE}
\lnorm \tp[-s] \frac{D_{\okos}(r^*\phi)}{r^*}(w')^{1/2}\rnorm_2^2 &\lesssim S_0[\phi](T).
\end{align}
\end{subequations}
The inequalities \eqref{STEA}-\eqref{STED} follow from the inequality, for $\epsilon > 0$,
\begin{equation}
\int_0^T \frac{E_0[\phi](t)}{(1+t)^{1+2\epsilon}}\, dt \lesssim_\epsilon E_0[\phi](T).
\end{equation}
 Additionally, for \eqref{STEA2}, we use $s-1-\gamma/2+\delta < -\frac12 - \delta,$ $\gamma/2 < 1/2 < s$, and \eqref{STED} follows from an application of H\"older's inequality, combined with the inequality $s-3/2+2\delta < -1/2$. Inequality \eqref{STEE} comes from our spacetime energy norm. Then it follows from \eqref{MetLI}, \eqref{STEA2} and \eqref{STED} that
\begin{equation}
\label{STEF}
\lnorm\tp[2s-1]H_1^{\gamma\delta}D_\gamma\phi\overline{D_\delta\phi} w\rnorm_1 \lesssim \varepsilon_g E_0[\phi](T),
\end{equation}
which will be useful later. We define the modified energy momentum tensor
\begin{equation}
\label{EMPhi}
\widetilde{T}[\phi]_{\alpha\beta} = \frac{1}{r^{*2}}\mathfrak{R}\left(D_\alpha(r^*\phi)\overline{D_\beta(r^*\phi)} - \frac12 \mhat_{\alpha\beta}\mhat^{\gamma\delta}D_\gamma(r^*\phi)\overline{D_\delta(r^*\phi)} \right).
\end{equation}

It follows that
\begin{equation}
\nabla_\mhat^\alpha \widetilde{T}[\phi]_{\alpha\beta} = -\tfrac{2\nabla_\mhat^\alpha(r^*)}{r^{*}}\widetilde{T}[\phi]_{\alpha\beta} + \tfrac{1}{r^{*2}}\mathfrak{R}\left(\Box_\mhat^{\mathbb{C}}(r^*\phi)\overline{D_\beta(r^*\phi)}\right) + \tfrac{1}{r^{*2}}\mathfrak{I}\left(r^*\phi \overline{D_{\mhat}^{\alpha}(r^*\phi)}\right)\bF_{\alpha\beta}.
\end{equation}

The identity \eqref{rBoxComm} gives
\[
\tfrac{1}{r^{*2}}\mathfrak{R}\left(\Box_\mhat^{\mathbb{C}}(r^*\phi)\overline{D_\beta(r^*\phi)}\right) = \tfrac{1}{r^{*2}}\mathfrak{R}\left(\left(r^*\Box_\mhat^{\mathbb{C}}\phi + r^{*2}\phi\Box_\mhat\left(\tfrac{1}{r^*}\right) + \tfrac{2\nabla_\mhat^\alpha(r^*)}{r^{*}}D_\alpha(r^*\phi)\right)\overline{D_\beta(r^*\phi)}\right).
\]
Combining these and taking the necessary cancellations gives us
\begin{equation}
\label{EMTDivPhi}
\nabla_\mhat^\alpha \widetilde{T}[\phi]_{\alpha\beta} = \tfrac{\nabla_\mhat^\alpha r^*}{r^{*3}}\mhat_{\alpha\beta}D_\gamma(r^*\phi)\overline{D_{\mhat}^\gamma(r^*\phi)} +\mathfrak{R}\left(\left(\Box_\mhat^{\mathbb{C}}\phi + r^{*}\phi\Box_\mhat\left(\tfrac{1}{r^*}\right)\right)\overline{\tfrac{D_\beta(r^*\phi)}{r^*}}\right) + \mathfrak{I}\left(\phi \tfrac{\overline{D_{\mhat}^{\alpha}(r^*\phi)}}{r^*}\right)\bF_{\alpha\beta}
\end{equation}
We look at these terms separately. Since $1/r^*$ is a fundamental solution of the wave operator with respect to $\mhat$ and $\okos(r^*)$ vanishes at 0, 
\begin{equation}
\mathfrak{R}\left( r^{*}\phi\Box_\mhat\left(\tfrac{1}{r^*}\right)\overline{\tfrac{D_\beta(r^*\phi)}{r^*}} \okos^\beta w\right) = 0.
\end{equation}

For $P^3$, we split $\bF = \bF^0  + \bF^1$. Then, $w \leq \tm w'$ in the support of $\bF^0$ so
\begin{equation}
\label{CurrentPhiCharge}
\lnorm\phi\tfrac{\overline{D_{\mhat}^\alpha(r^*\phi)}}{r^*}\bF^0_{\alpha\beta}\okos^\beta w \rnorm_1 \lesssim \lnorm\tp[s-1]\tz[1/2+\overline{\mu}]\phi (w')^{1/2}\rnorm_2\lnorm\tp[2-s]\tz[1/2-\overline{\mu}]\tfrac{D_{\mhat}^\alpha(r^*\phi)}{r^*}\bF^0_{\alpha\beta}\okos^\beta(w')^{1/2}\rnorm_2.
\end{equation}
The first term on the right is easily bounded by $\mathcal{E}[\phi]^{1/2}$. Applying \eqref{ChargeLInfty} and expanding in the null frame gives
\begin{equation}
\left|\tfrac{D_{\mhat}^\alpha(r^*\phi)}{r^*}\bF^0_{\alpha\beta}\okos^\beta\right| \lesssim |q|\left(\left|\tp[2s-2]\tfrac{D_{\Ls}(r^*\phi)}{r^*}\right|  + \left|\tm[2s]\tp[-2]\tfrac{D_{\uLs}(r^*\phi)}{r^*}\right|\right).
\end{equation}
We can plug these in to \eqref{CurrentPhiCharge}, noting $2\overline{\mu} < s$, to see that
\begin{equation}\label{EEstPhiF0}
\lnorm\phi\tfrac{\overline{D_{\mhat}^\alpha(r^*\phi)}}{r^*}\bF^0_{\alpha\beta}\okos^\beta w \rnorm_1 \lesssim |q|\mathcal{E}_0[\phi](T).
\end{equation}
We have some room in this estimate along the light cone, but it is sharp with regards to spatial decay. In order to handle $\bF^1$ we first take
\begin{equation}
\label{CurrentPhiRem}
\lnorm\phi\tfrac{\overline{D_{\mhat}^\alpha(r^*\phi)}}{r^*}\bF^1_{\alpha\beta}\okos^\beta w \rnorm_1 \lesssim \lnorm\tp[s-3/2-\delta]\phi w^{1/2}\rnorm_2\lnorm\tp[3/2+\delta-s]\tfrac{D_{\mhat}^\alpha(r^*\phi)}{r^*}\bF^1_{\alpha\beta}\okos^\beta w^{1/2}\rnorm_2.
\end{equation}
We have the bound
\begin{equation}
\left|\tfrac{D_{\mhat}^\alpha(r^*\phi)}{r^*}\bF^1_{\alpha\beta}\okos^\beta\right| \lesssim \lVert \bF^1\rVert^{red}_{L^{\infty}[w]}\left(\left|\tp[s-1]\tm[-1/2]\tfrac{D_{\Ls}(r^*\phi)}{r^*}\right| + \left|\tp[s-3/2]\tfrac{\slashed{D}(r^*\phi)}{r^*}\right|+ \left|\tp[-1-s]\tm[2s-1/2]\tfrac{D_{\uLs}(r^*\phi)}{r^*}\right|\right)
\end{equation}
Combining this with \eqref{CurrentPhiRem} and \eqref{EEstPhiF0} gives
\begin{equation}\label{EEstPhiF}
\lnorm\phi\tfrac{\overline{D_{\mhat}^\alpha(r^*\phi)}}{r^*}\bF_{\alpha\beta}\okos^\beta w \rnorm_1 \lesssim (|q| + \lVert \bF^1\rVert^{red}_{L^{\infty}[w]})\mathcal{E}_0[\phi](T).
\end{equation}

Next we look at the deformation tensor with respect to $\mhat$. We recall the identity
\begin{equation}\label{DTStatement}
\text{symm }\nabla_\mhat^\alpha \okos^\beta = \tfrac12 \tfrac{\uls^{2s} - \abus^{2s}}{r^*}\mhat^{\alpha\beta} + \tfrac14(\tfrac{\uls^{2s} - \abus^{2s}}{r^*} - 2s(\uls^{2s-1} + \us\abus^{2s-2}))(\Ls^\alpha\uLs^\beta + \Ls^\beta\uLs^\alpha),
\end{equation}
We are now ready to state our first result.
\begin{Lemma}
Define $\mathcal{E}_0^+ = E_0[\phi](T) + S_0[\phi](T) +  C_0^+[\phi](T)$ 
Given a function $\phi$, for sufficiently small $M$ we have the inequality
\begin{align}
\label{FirstEEPhi}
\mathcal{E}_0^+[\phi](T) &\lesssim  \mathcal{E}_0[\phi](0) + \left(|q| + \lVert \bF^1 \rVert^{red}_{L^{\infty}[w]}\right)\mathcal{E}_0[\phi](T) + \left|\int_{[0,T]\times \Sigma_t}\Box_\mhat^\mathbb{C}\phi \tfrac{\overline{D_{\okos}(r^*\phi)}}{r^*}w\right| + \\
&+ \left|\int_{[0,T]\times \Sigma_t \backslash \{C_{max}\}}\Box_{\mhat}^\mathbb{C}\phi \tfrac{\overline{D_{\okos}(r^*\phi)}}{r^*}w\right|\nonumber
\end{align}
\end{Lemma}
The domain of the last integral, containing $\{C_{max}\}$, is the integral outside the light cone corresponding to our $C_0$ energy.

\begin{proof}
This follows from an application of the divergence theorem over time slabs (and over the reduced slabs $[0,T] \times \{\us \leq C\}$.) 

We have that
\begin{equation}\label{id:PhiDivergence}
-\nabla_\mhat^\alpha \left(\widetilde{T}[\phi]_{\alpha\beta}\okos^\beta \widetilde{w}\right) = - (\nabla_\mhat^{\alpha}\okos^\beta) \widetilde{T}_{\alpha\beta}\wt{w} - \okos^\beta\nabla_\mhat^\alpha\wt{T}_{\alpha\beta}\wt{w} - (\nabla_\mhat \wt{w})^\alpha \okos^\beta \wt{T}_{\alpha\beta}
\end{equation}
Expanding out the initial data norms at $t = 0, t = T$ almost immediately gives us $E_0$ (up to a equivalence), with the expression \eqref{TSEnergyPhiE}.

We may symmetrize the first term on the right hand side of \eqref{id:PhiDivergence}. Then, \eqref{DTStatement}
We combine this with the identity \eqref{EMTDivPhi}, noting first that
\[
\tfrac{\nabla_\mhat^\alpha r^*}{r^{*3}}\okos^\beta\mhat_{\alpha\beta} = \frac12(\uls^{2s} - \abus^{2s}), \qquad \text{tr}_{\mhat}\wt{T} = -\frac{1}{r^{*2}}D_\alpha(r^*\phi)D^\alpha(r^*\phi).
\]
Therefore,by \eqref{Lemma32}, 
\begin{equation}
-\nabla_\mhat^\alpha \left(\widetilde{T}[\phi]_{\alpha\beta}\okos^\beta \widetilde{w}\right) \leq -\tfrac{1}{r^{*2}}\mathfrak{R}\left(\Box_\mhat^{\mathbb{C}}(r^*\phi)\overline{D_{\okos}(r^*\phi)}\right) - \tfrac{1}{r^{*2}}\mathfrak{I}\left(r^*\phi \overline{D_{\mhat}^{\alpha}(r^*\phi)}\right)\bF_{\alpha\beta}\okos^\beta- (\nabla_\mhat \wt{w})^\alpha \okos^\beta \wt{T}_{\alpha\beta}.
\end{equation}
The first term appears in the right hand side of \eqref{FirstEEPhi}, and the second term can be bounded using \eqref{EEstPhiF}. It now suffices to prove that we may include $S_0$ and $C_0^+$ in our energy.
When the derivative falls on $\widetilde{w}$, we take the null decomposition
\begin{equation}
\nabla^\alpha(\widetilde{w}) = \Ls^{\alpha}\mhat^{\Ls\uLs}\uLs(\widetilde{w}) + \uLs^\alpha \mhat^{\uLs\Ls}\Ls(\widetilde{w})
\end{equation}
The first term is equivalent to $\Ls^{\alpha}w'$, and the second term is equivalent to  
$\uLs^\alpha\tz[1+2\overline{\mu}]w'$. Expanding out $\wt{T}$ in the null decomposition and integrating gives an integral equivalent to $-S_0$ on the right (after applying the Hardy estimate \eqref{HardyEstimate}), which we may move over to the left hand side.

 In order to bound $C_0^+$, we repeat the application of the divergence theorem, now over the exterior of the light cone where $C_0^+$ attains its maximum.
 \end{proof}
We now bound the perturbations on this energy estimate which arise from the metric.
\begin{Lemma}
\label{RemainderDivergence}
Defining
\begin{equation}
C_{err}[\phi]= \sup_{\us}\int_{C_{\us}}\partial_\beta(\us)\tilde{Q}[\phi]_{\okos}^\beta w,
\end{equation}
where $\partial_\beta(\us)\tilde{Q}[\phi]_{\okos}^\beta$ is defined in \eqref{RTensorF},
The following inequality holds for any function $\phi$:
\begin{align}
\left|\int_{[0,T] \times \Sigma_t}\mathfrak{R}\left(\left(\Box_g^{\mathbb{C}}\phi - \Box_\mhat^{\mathbb{C}}\phi\right)\tfrac{\overline{D_{\okos}(r^*\phi)}}{r^*} w\right)\, dx \, dt\right| + & \\
\left|\int_{[0,T] \times \Sigma_t \backslash \{C_{max}\}}\mathfrak{R}\left(\left(\Box_g^{\mathbb{C}}\phi - \Box_\mhat^{\mathbb{C}}\phi\right)\tfrac{\overline{D_{\okos}(r^*\phi)}}{r^*} w\right)\, dx \, dt\right|& \lesssim \epsilon E[\phi](1+\lnorm F \rnorm_{L^\infty[w]}) + C_{err}[\phi].
\end{align}
\end{Lemma}
\begin{proof}
For each integral, we split this up into two parts. Defining the reduced derivative 
\[
\wt{D}_\alpha = \partial_\alpha + iA_\alpha,
\]
we define 
\begin{equation}
\wt\Box^{\mathbb{C}}_\mhat\phi  = \mhat^{\alpha\beta}\wt{D}_\alpha\wt{D}_\beta\phi.
\end{equation}
Then, we take
\begin{equation}
\Box^{\mathbb{C}}_g\phi  - \Box^{\mathbb{C}}_\mhat\phi = (\Box^{\mathbb{C}}_g\phi  - \wt\Box^{\mathbb{C}}_\mhat\phi) + (\wt\Box^{\mathbb{C}}_\mhat\phi  - \Box^{\mathbb{C}}_\mhat\phi)
\end{equation}
We will use the harmonic coordinate condition to bound the first term on the right hand side. The second term can be written in terms of the rapidly decaying Christoffel symbols of $\mhat$ with respect to the background Minkowski metric.


Therefore, by the inequalities $M < \epsilon$, and \eqref{STEA} and \eqref{STEE}, we have
\begin{equation}
\lnorm\left(m^{*\alpha\beta}\tilde{D}_\alpha\tilde{D}_\beta\phi - \Box_{m^*}^{\mathbb{C}}\phi\right)\frac{\overline{D_{\okos}(r^*\phi)}}{r^*} w\rnorm_1 \lesssim\epsilon E[\phi]
\end{equation}

Next we want to bound the quantity
\begin{equation}
\label{BoxRemainder}
\int_0^T\intsig{t}\widetilde{H}^{\alpha\beta}\tilde{D}_\alpha\tilde{D}_\beta\phi\frac{\overline{D_{\okos}(r^*\phi)}}{r^*}w \, dx \, dt
\end{equation}


We define the remainder momentum density tensor
\begin{equation}
\label{RTensorF}
\tilde{Q}[\phi]_{\okos}^\beta = \mathfrak{R}\left(\frac{\overline{D_{\okos}(r^*\phi)}}{r^*} \widetilde{H}^{\beta\gamma}D_\gamma\phi - \frac12 \okos^\beta \widetilde{H}^{\gamma\delta}D_\gamma\phi\overline{D_\delta\phi}\right).
\end{equation}
and apply the divergence theorem to this quantity in Euclidean space, in which we can ignore the distinction between $D$ and $\tilde{D}$. As usual, we conduct our analysis in the extended exterior $r > \frac{t}{2}$, as we can use uniform estimates for the interior. We have by the divergence theorem
\begin{equation}
\int_0^T\intsig{t}\partial_\beta\left(\tilde{Q}[\phi]_{\okos}^\beta \widetilde{w}\right) \, dx \, dt = \intsig{T}\tilde{Q}[\phi]_{\okos}^0 \widetilde{w}\, dx - \intsig{0}\tilde{Q}[\phi]_{\okos}^0. \widetilde{w} \, dx
\end{equation}
Our goal here is to isolate the desired quantity, \eqref{BoxRemainder}, on the left hand side and move the rest, including the time-slice integrals, over to the right hand side, where we bound these quantities using the energy.

 When the derivative falls on $\phi$ or $D\phi$, we get
\[
\mathfrak{R}\left(\frac{\overline{D_{\okos}(r^*\phi)}}{r^*}\widetilde{H}^{\beta\gamma}D_\beta D_\gamma\phi\right) + \frac{\okos(r^*)}{r^*}\widetilde{H}^{\beta\gamma}D_\gamma\phi\overline{D_\beta\phi} + \mathfrak{R}\left(F_{\beta \okos}\phi H^{\beta\gamma}\overline{D_\gamma\phi}\right).
\]
The first term is precisely what we are looking for, and the second term can be bounded in the $L^1$ spacetime norm using \eqref{STEF}. We now look at the third term. We note that
\begin{subequations}
\begin{align}
|F_{\uLs\okos}| &\lesssim \tp[-1+s]\tm[-1+s]\lnorm F\rnorm_{L^\infty[w]}, \\
|F_{\Bs{j}\okos}| &\lesssim \tp[-3/2+s]\tm[-1/2+s]\lnorm F\rnorm_{L^\infty[w]}, \\
|F_{\Ls\okos}| &\lesssim \tp[-1-s]\tm[-1+3s]\lnorm F\rnorm_{L^\infty[w]}.
\end{align}
\end{subequations}
Expanding in the null frame and combining this with the bounds
\begin{subequations}
\begin{align}
\epsilon\left\lVert\tm[-1/2+s]\tp[-3/2+s-1+\delta]\phi D\phi w\right\rVert_1 &\lesssim \epsilon\lnorm\tp[-1]\phi w^{1/2}\rnorm_2\lnorm\tp[-1/2-\delta]\tm[s]D\phi w^{1/2}\rnorm_2, \\
\epsilon\left\lVert\tm[-1+s]\tp[-1+s-1+\delta]\phi \overline{D}\phi w\right\rVert_1 &\lesssim \epsilon\lnorm\tp[-1]\phi w^{1/2}\rnorm_2\lnorm\tp[s-1+\delta]\overline{D}\phi w^{1/2}\rnorm_2,\\
\epsilon\left\lVert\tm[-1+s+\gamma']\tp[-1+s-1 - \gamma' +\delta]\phi D\phi w\right\rVert_1 &\lesssim \epsilon\lnorm\tp[-1]\phi w^{1/2}\rnorm_2\lnorm\tp[-1-\delta]\tm[s]D\phi w^{1/2}\rnorm_2,
\end{align}
\end{subequations}
gives us the uniform bound
\[
\left|\mathfrak{R}\left(F_{\beta \okos}\phi H^{\beta\gamma}\overline{D_\gamma\phi}\right)\right| \lesssim\epsilon E[\phi](\lnorm F \rnorm_{L^\infty[w]}).
\]
Now we look at when the derivative falls on metric terms of \eqref{RTensorF}. We have the estimates
\begin{subequations}
\begin{align}
\left|(\partial_\beta \widetilde{H}^{\beta\gamma})D_\gamma\phi\right| &\lesssim \epsilon\left(\tp[-1-\gamma'+\delta]\tm[\gamma'-1]|D\phi| + \tp[-1+\delta]\tm[-1]|\overline{D}\phi|\right) \\
\left|\okos(\widetilde{H}^{\gamma\delta})D_\gamma\phi\overline{D_\delta\phi}\right| &\lesssim \epsilon\left(\tp[2s-2-\gamma'+\delta]\tm[\gamma']|D\phi|^2 + \tp[2s-2+\delta]|D\phi||\overline{D}\phi|\right)
\end{align}
\end{subequations}
from which follow
\small
\begin{subequations}
\begin{align}
\lnorm\frac{\overline{D_{\okos}(r^*\phi)}}{r^*} (\partial_\beta\widetilde{H}^{\beta\gamma})D_\gamma\phi w\rnorm_1 &\lesssim \epsilon \lnorm \tp[-s]\tm[-1/2-\delta]\frac{D_{\okos}(r^*\phi)}{r^*}w^{1/2}\rnorm_2\left(\lnorm\tp[-1-\delta]\tm[1/2]|D\phi|w^{1/2}\rnorm_2 + \lnorm\tp[s-1/2-\delta]|\overline{D}\phi|w^{1/2}\rnorm_2\right) \\
\lnorm\okos(H^{\gamma\delta})D_\gamma\phi\overline{D_\delta\phi}w\rnorm_1&\lesssim \epsilon \left(\lnorm\tp[-1/2-\delta]\tm[s]|D\phi|w^{1/2}\rnorm_2^2 + \lnorm\tp[2s-1/2-\delta]|\overline{D}\phi|\rnorm_2 \lnorm\tp[-1/2-\delta]|D\phi|w^{1/2}\rnorm_2\right)
\end{align}
\end{subequations}
\normalsize
where the last estimate comes from H\"older's inequality and the condition $s - 4\delta > 1/2$. The inequality follows.

Next, we consider the case where the derivative falls on $\okos$. This is fortunately more straightforward, since for most terms which appear we do not need to differentiate derivatives. We have the terms
\begin{equation}
\mathfrak{R}\left(\widetilde{H}^{\beta\gamma}\partial_\beta\left(\frac{\okos(r^*)}{r^*}\right)\overline{\phi}D_\gamma\phi - \frac12(\partial_\beta\okos^\beta)H^{\gamma\delta}D_\gamma\phi\overline{D_\delta\phi} + (\partial_\beta\okos^\alpha)\overline{D_\alpha\phi}\widetilde{H}^{\alpha\beta}D_\beta\phi\right).
\end{equation}
We can bound the first two terms on the right by
\begin{subequations}
\begin{align}
\left\lVert\widetilde{H}^{\beta\gamma}\partial_\beta\left(\frac{\okos(r^*)}{r^*}\right)\overline{\phi}D_\gamma\phi w\right\rVert_1 &\lesssim \epsilon\lnorm\tp[2s-3+\delta]|\phi||D\phi| w\rnorm_1, \\
&\lesssim \epsilon \lnorm\tp[s-3/2-\delta]|\phi| w^{1/2}\rnorm_2\lnorm\tp[s-3/2+2\delta]|D\phi|w^{1/2}\rnorm_2,\nonumber \\
\lnorm(\partial_\beta\okos^\beta)H^{\gamma\delta}D_\gamma\phi\overline{D_\delta\phi} w \rnorm_1 &\lesssim \epsilon\left(\lnorm\tp[2s-2+\delta]|D\phi||\overline{D}\phi|w\rnorm_1 + \lnorm\tp[2s-2-\gamma'+\delta]\tm[\gamma']|D\phi|^2w\rnorm_1\right).
\end{align}
\end{subequations}
Both of these fit in our energy norm as a direct consequence of \eqref{STEnergy}. For the third term, in the exterior we have the terms
\begin{subequations}
\begin{align}
|B_j(\okos^\alpha)D_\alpha\phi| &\lesssim |\tp[2s-1]D_{B_j}\phi|, \\
|\Ls(\okos^\alpha)D_\alpha\phi| &\lesssim |\tp[2s-1]D_{\Ls}\phi| + |\tm[2s]\tp[-1]D_{\uLs}\phi|, \\
|\uLs(\okos^\alpha)D_\alpha\phi| &\lesssim \tp[2s-1]|D\phi|.
\end{align}
\end{subequations}
Thus,
\begin{equation}
\left|\partial_\beta\okos^\alpha)\overline{D_\alpha\phi}\widetilde{H}^{\alpha\beta}D_\beta\phi\right| \lesssim \epsilon\left(\tp[2s-2+\delta]|\overline{D}\phi||D\phi| + \tm[2s]\tp[-2+\delta]|D\phi|^2 + \tm[\gamma']\tp[2s-2-\gamma'+\delta]|D\phi|^2\right).
\end{equation}
The $L^1$ norms corresponding to these terms are therefore contained in our energy norm.

Finally, we look at the case when the derivative falls on $\widetilde{w}$. We don't have any nice sign condition, so we use the pointwise estimates
\small
\begin{align}
\lnorm\tilde{Q}[\phi]_{\okos}^\beta \partial_\beta w\rnorm & \lesssim \epsilon\lnorm\tp[-s]\tm[-1/2-\delta]\frac{D_{\okos}(r^*\phi)}{r^*}w^{1/2}\rnorm_2\left(\lnorm\tp[s-1-\gamma'+\delta]\tm[1/2+\delta]|D\phi| w^{1/2}\rnorm_2 + \lnorm\tp[s-1+\delta]\tm[1/2+\delta-1]|\overline{D}\phi|w^{1/2}\rnorm_2\right) +\nonumber\\
&\quad+\epsilon\lnorm\tp[2s-2+\delta]|D\phi||\overline{D}\phi|w\rnorm_1 + \epsilon\lnorm\tp[2s-2-\gamma'+\delta]\tm[\gamma']|D\phi|^2w\rnorm_1.
\end{align}
\normalsize
By the norms in \eqref{STEnergy}, the right hand side can be bounded by $\epsilon E[\phi](T)$.
\end{proof}




==> ChJuly/MetricAssumptionsJuly.tex <==
One advantage of the null frame of the previous section over the standard null frame in Minkowski space is that we can for the most part treat the sum of the Minkowski and ADM parts of the metric as a unified quantity, which models the background geometry. This is in contrast to \cite{LR10}, which treated the ADM part as an error term.

We split $g_{\alpha\beta} = \mt_{\alpha\beta} + h_{\alpha\beta}$, $g^{\alpha\beta} = (\mt^{-1})^{\alpha\beta} + H^{\alpha\beta}$, where
\begin{equation}
\mt_{\alpha\beta} = m_{\alpha\beta} + \frac{M\chi}{r}\delta_{\alpha\beta}.
\end{equation}
with all other components equal to 0. We define $(\mt^{-1})$ to be the inverse metric of $\mt$, and note that $h_{\alpha\beta}= -H_{\alpha\beta} + O(|h|^2)$. We note that
\[
|\mt_{\Ls\Ls}|+|\mt_{\Ls \Bs{j}}| \lesssim M\tp[-2]
\]
everywhere except in the far interior (in particular, the region where $\partial\chi \neq 0$). In the far interior, $\mt_{\Ls\Ls}$ decays like $M\tp[-1+\delta']$, which in this region is bounded above by a constant times $M\tm[1+\delta']\tp[-2]$. We can consider the latter as a uniform bound.

Now we look at $H$. Since we are for now treating this as a modular estimate for the full EMKG system, we assume $L^\infty$ estimates on low derivatives of $H$ and $L^2$ estimates on high derivatives of $H$ as follows: We first consider $\gamma' < \gamma < 1$. Then, we define the class $G_{\epsilon_g, \gamma', \gamma, k}$ to be the set of metrics $g$ with $M \leq \epsilon_g$ (where $M$ is the multiplier corresponding to the ADM part of the metric) satisfying the $L^\infty$ norms
\begin{subequations}
\label{MetLI}
\begin{align}
 M &< \epsilon_g, \\
|\Lie{X}^Ih| &< \epsilon_g\tp[-1+\delta'], \\
|\Lie{X}^I h|_{\mcL\mcT} &< \epsilon_g\tz[\gamma']\tp[-1+\delta'],
\end{align}
\end{subequations}
for a multiindex $I, |I| \leq k - 6$, and $X \in \mathbb{L}$, and
\begin{subequations}
\label{MetL2}
\begin{align}
\label{L21}
\left\lVert|\partial\Lie{X}^Ih|w_g^{1/2}\right\rVert_{L^2(\mathbb{R}^3)} + \left\lVert\tm[-1]|\Lie{X}^Ih|w_g^{1/2}\right\rVert_{L^2(\mathbb{R}^3)}&\leq \epsilon_g (1+t)^{\delta/2}, \\
\label{L22}
\left\lVert\tm[-1/2-\delta]\big(|\partial\Lie{X}^Ih|_{\Ls\Ls}+ |\overline\partial\Lie{X}^Ih|\big) w_g^{1/2}\right\rVert_{L^2([0,T]\times\mathbb{R}^3)} + \left\lVert\tm[-3/2-\delta]|\Lie{X}^Ih|_{\Ls\Ls}w_g^{1/2}\right\rVert_{L^2([0,T]\times\mathbb{R}^3)}&\leq \epsilon_g(1+T)^{\delta'/2},
\end{align}
\end{subequations}
for $|I| \leq k$, some small constant $\delta' > 0$ ,and
\begin{equation}
w_g = \begin{cases}
1 & r^* \leq t, \\
1 + (r^* - t)^{1+2\gamma} & r^* \geq t.
\end{cases}
\end{equation}

We note that in equations \eqref{L21} and \eqref{L22}, the bound for the second norm on the left follows from \eqref{Hardy1} and \eqref{Hardy2}. As a note, the required weight is higher than in \cite{LR10}, and thus we require more initial decay; this is consistent with the additional $L^\infty$ decay required near the light cone.

 In general, $k\geq 11$, and $1/2 + 4\delta' < \gamma' < \gamma - 4\delta' < \gamma < 1 - 4\delta'$. Finally, we assume the initial conditions that at time $t = 0$, we have a split metric, with
\begin{equation}
g_{00} = -\left(1-\frac{M\chi}{r}\right), \qquad g_{0i} = 0
\end{equation}
In the spacetime integrals the value of $\tm$ on the left is that corresponding to the integrated time variable $\tau$. These are consistent with estimates established in \cite{LR10} and \cite{L15}, where we use the weak null condition for the spacetime estimates on the $\Ls\Ls$ terms. These will in particular be useful when taking commutators.

We have analogous estimates on components of the raised metric. In particular, if we write out the matrix $g_{X_iX_j}$, where $X_i, X_j$ are elements in our null frame, and then take the inverse by adjoints, we see that every error term appearing in $g^{\uLs\uLs}, g^{\uLs\Bs{}}$ contains either a term decaying like $\tm[\gamma']\tp[-1-\gamma'+\delta']$ or $\tp[-2+2\delta']$. We therefore have the estimates
\begin{subequations}
\label{RMetric}
\begin{align}
|g^{\uLs\uLs}| + |g^{\uLs\Bs{i}}| &\lesssim \epsilon_g\tm[\gamma']\tp[-1-\gamma'+\delta], \\
\left|g^{\Ls\uLs} + \frac12\right| + \left|g^{\Bs{i}\Bs{i}} - 1\right| &\lesssim \epsilon_g\tp[-1+\delta], \\
|g^{\Ls\Ls}| + |g^{\Bs{1}\Bs{2}}|+ |g^{\Ls\Bs{i}}| &\lesssim \epsilon_g\tp[-1+\delta].
\end{align}
\end{subequations}

We can therefore prove the following lemma:
\begin{Lemma}
\label{RaisedEst}
Given a two-tensor $T_{\alpha\beta}$, we can define the following norms:
\begin{equation}
|T| = |T|_{\mcU\mcU}, |\slashed{T}| = |T|_{\mcT\mcT} + |T|_{\mcL\mcU} + |T|_{\mcU\mcL},
\end{equation}
where we recall $\mcL = \{\Ls\}, \mcT = \{\Ls, \{\Bs{i}\}\}, \mcU = \{\Ls, \uLs, \{\Bs{i}\}\}$ and each norm denotes the sum of the norms for each field in the sets $\mcL, \mcU, \mcT$. Then, we have the following estimates on the raised components $T^{XY}$:
\begin{subequations}
\begin{align}
\left|T^{\uLs\uLs} - \frac14T_{\Ls\Ls}\right|  &\lesssim \epsilon_g\left(\tp[-1+\delta']|T_{\mcL\mcL}| + \tm[\gamma]\tp[-1-\gamma'+\delta']|\slashed{T}| + \tm[2\gamma']\tp[-2-2\gamma'+2\delta']|T|\right), \\
\label{ExampleRaised}
\left|T^{\uLs\Bs{j}} + \frac12T_{\Ls\Bs{j}}\right| + \left|T^{\Bs{j}\uLs} + \frac12T_{\Bs{j}\Ls}\right| &\lesssim \epsilon_g\left(\tp[-1+\delta'](|T_{\mcL\mcT}| + |T_{\mcT\mcL}|) + \tm[\gamma']\tp[-1-\gamma'+\delta']|T|\right), \\
\left|T^{\uLs\Ls} - \frac14T_{\Ls\uLs}\right| + \left|T^{\Ls\uLs} - \frac14T_{\uLs\Ls}\right| &\lesssim \epsilon_g\left(\tp[-1+\delta']|\slashed{T}| + \tm[\gamma']\tp[-1-\gamma'+\delta']|T|\right), \\
\left|T^{\Bs{i}\Bs{j}} - T_{\Bs{i}\Bs{j}}\right|  &\lesssim \epsilon_g\left(\tp[-1+\delta']|\slashed{T}| + \tm[\gamma']\tp[-1-\gamma'+\delta']|T|\right), \\
\left|T^{\Ls\Bs{j}} + \frac12 T_{\uLs\Bs{j}}\right| + \left|T^{\Bs{j}\Ls} + \frac12 T_{\Bs{j}\uLs}\right| &\lesssim \epsilon_g\tp[-1+\delta']|T|, \\
\left|T^{\Ls\Ls} - \frac14 T_{\uLs\uLs}\right|  &\lesssim \epsilon_g\tp[-1+\delta']|T|
\end{align}
\end{subequations}
\end{Lemma}
\begin{proof}
This almost entirely follows from equation \eqref{RMetric}. As an example, we prove our result for the first term on the left hand side of equation \eqref{ExampleRaised}. We first rewrite
\begin{equation}
T^{\uLs\Bs{j}} = \sum_{\substack{ X,Y \in \mcU}} g^{\uLs X}T_{XY}g^{Y\Bs{j}}
\end{equation}
If $X = \Ls$ and $Y = \Bs{j}$, we have the term which is subtracted off plus an error term which is directly bounded by the first term on the right hand side. If $X = \Ls$ and $Y = \Ls$ or $\Bs{i}$, we likewise have something bounded by the first term on the right. If $X = \Ls$ and $Y = \uLs$, we have a term like $g^{\uLs\Bs{j}}$, which has our better decay norm.
If $X \neq \Ls$, we likewise have either $g^{\uLs\uLs}$ or $g^{\uLs\Bs{i}}$, both of which have our better decay norms. Other component estimates follow similarly.
\end{proof}

Now we define a vector which will be useful in the energy estimate:
\begin{equation}
\Lt = \nabla \us,
\end{equation}
the normal vector to surfaces of constant $\us$. We note that $\Lt$ is very close to a scalar multiple of $L$, in the sense that
\[
g_{\Lt\Ls}, g_{\Lt S_j^*} = 0,
\]
which is a restatement of the relations $\Ls(\us), \Bs{j}(\us) = 0$. We know that the $\uLs$ component of $\Lt$ in the modified null decomposition is bounded by $C\epsilon\tm[\gamma']\tp[-1-\gamma'+\delta]$. This will be useful later, as we can bound error terms from the metric using an integrated $L^\infty$ estimate, at the expense of requiring more derivatives of the function in the energy.


==> ChJuly/MetricAssumptionsJulyHansSuggestion.tex <==
One advantage of the null frame of the previous section over the standard null frame in Minkowski space is that we can for the most part treat the sum of the Minkowski and ADM parts of the metric as a unified quantity, which models the background geometry. This is in contrast to \cite{LR10}, which treated the ADM part as an error term.

We split $g_{\alpha\beta} = \mt_{\alpha\beta} + h_{\alpha\beta}$, $g^{\alpha\beta} = (\mt^{-1})^{\alpha\beta} - H^{\alpha\beta}$, where
\begin{equation}
\mt_{\alpha\beta} = m_{\alpha\beta} + \frac{M\chi}{1+r}\delta_{\alpha\beta}.
\end{equation}
with all other components equal to 0. Note that $(\mt^{-1})$ here is the inverse metric of $\mt$. This use is identical to that in \cite{LR}. We note that
\[
\mt_{\Ls\Ls}, \mt_{\Ls \Bs{j}} \approx M\tp[-2]
\]
everywhere except in the far interior (in particular, the region where $\partial\chi \neq 0$). In the far interior, $\mt_{\Ls\Ls}$ decays like $M\tp[-1+\delta']$, which we can in particular rewrite as $M\tm[1+\delta']\tp[-2]$. We can consider the latter as a uniform bound.

Now we look at $H$. Since we are for now treating this as a model estimate for the full EMKG system, we assume $L^\infty$ estimates on low derivatives of $H$ and $L^2$ estimates on high derivatives of $H$ as follows: We first consider $\gamma' < \gamma < 1$. Then, we define the class $G_{\epsilon, \gamma', \gamma, k}$ to be the set of metrics $g$ with $M \leq \epsilon$ (where $M$ is the multiplier corresponding to the ADM part of the metric) satisfying the $L^\infty$ norms
\begin{subequations}
\label{MetLI}
\begin{align}
 M &< \epsilon, \\
|\Lie{\mathbb{L}}^Ih| &< \epsilon\tp[-1+\delta'], \\
|(\Lie{\mathbb{L}}^I h)_{\mcL\mcT}| &< \epsilon\tm[\gamma']\tp[-\gamma'-1+\delta'],
\end{align}
\end{subequations}
for a multiindex $I, |I| \leq k - 6$, and $X \in \mathbb{L}$, and 
\begin{subequations}
\label{MetL2}
\begin{align}
\label{L21}
\left\lVert|\partial\Lie{X}^Ih|w_1^{1/2}\right\rVert_{L^2(\mathbb{R}^3)} + \left\lVert\tm[-1]|\Lie{X}^Ih|w_1^{1/2}\right\rVert_{L^2(\mathbb{R}^3)}&\leq \epsilon (1+t)^{\delta'/2}, \\
\label{L22}
\left\lVert\tm[-1/2]|(\partial\Lie{X}^Ih)_{\mcL\mcL}|+ |\overline\partial\Lie{X}^Ih|) w_1^{1/2}\right\rVert_{L^2([0,T]\times\mathbb{R}^3)} + \left\lVert\tm[-3/2]|(\Lie{X}^Ih)_{\mcL\mcL}|w_1^{1/2}\right\rVert_{L^2([0,T]\times\mathbb{R}^3)}&\leq \epsilon(1+t)^{\delta'/2},
\end{align}
\end{subequations}
for $|I| \leq k$, some small constant $\delta' > 0$ ,and
\begin{equation}
w_1 = \begin{cases}
1 & r^* \leq t, \\
1 + (r^* - t)^{1+2\gamma} & r^* \geq t.
\end{cases}
\end{equation}

We note that in each equation, the bound for the second term on the right follows from \eqref{Hardy1} and \eqref{Hardy2}. As a note, the required weight is higher than in \cite{LR}, and thus we require more initial decay; this is consistent with the additional $L^\infty$ decay required near the light cone.

We note that in general $\delta'$ scales like $C\epsilon$, for some uniform constant $C$.

 In general, $k\geq 11$, and $1/2 + 4\delta' < \gamma' < 1 - 4\delta'$. Finally, we assume the initial conditions that at time $t = 0$, we have a split metric, with
\begin{equation}
g_{00} = -\left(1-\frac{M\chi}{1+r}\right), \qquad g_{0i} = 0
\end{equation}
In the spacetime integrals the value of $\tm$ on the left is that corresponding to the integrated time variable $\tau$. These are consistent with estimates established in \cite{LR} and \cite{L15}, where we use the weak null condition for the spacetime estimates on the $\mcL\mcL$ terms. These will in particular be useful when taking commutators. 

We have analogous estimates on components of the raised metric. In particular, if we write out the matrix $g_{X_iX_j}$, where $X_i, X_j$ are elements in our null frame, and then take the inverse via the adjoint method, we see that every term appearing in $g^{\uLs\uLs}, g^{\uLs\Bs{}}$ contains either a term decaying like $\tm[\gamma']\tp[-1-\gamma'+\delta']$ or $\tp[-2+2\delta']$. We therefore have the estimates
\begin{subequations}
\label{RMetric}
\begin{align}
|g^{\uLs\uLs}| + |g^{\uLs\Bs{}}| &\lesssim \epsilon\tm[\gamma']\tp[-1-\gamma'+\delta'], \\
\left|g^{\Ls\uLs} + \frac12\right| + \left|g^{\Bs{i}\Bs{i}} - 1\right| &\lesssim \epsilon\tp[-1+\delta'], \\
|g^{\Ls\Ls}| + |g^{\Bs{1}\Bs{2}}|+ |g^{\Ls\Bs{}}| &\lesssim \epsilon\tp[-1+\delta'].
\end{align}
\end{subequations}

We can therefore prove the following lemma:
\begin{Lemma}
\label{RaisedEst}
Given a two-tensor $T_{\alpha\beta}$, we can define the following norms:
\begin{equation}
|T| = |T_{\mcU\mcU}|, |\slashed{T}| = |T_{\mcT\mcT}| + |T_{\mcL\mcU}| + |T_{\mcU\mcL}|,
\end{equation}
where we recall $\mcL = \{\Ls\}, \mcT = \{\Ls, \Bs{}\}, \mcU = \{\Ls, \uLs, \Bs{}\}$ and each norm denotes the sum of the norms for each field in the sets $\mcL, \mcU, \mcT$. Then, we have the following estimates on the raised components $T^{XY}$:
\begin{subequations}
\begin{align}
\left|T^{\uLs\uLs} - \frac14T_{\Ls\Ls}\right|  &\lesssim \epsilon\left(\tp[-1+\delta']|T_{\mcL\mcL}| + \tm[\gamma]\tp[-1-\gamma'+\delta']|\slashed{T}| + \tm[2\gamma']\tp[-2-2\gamma'+2\delta']|T|\right), \\
\label{ExampleRaised}
\left|T^{\uLs\Bs{j}} + \frac12T_{\Ls\Bs{j}}\right| + \left|T^{\Bs{j}\uLs} + \frac12T_{\Bs{j}\Ls}\right| &\lesssim \epsilon\left(\tp[-1+\delta'](|T_{\mcL\mcT}| + |T_{\mcT\mcL}|) + \tm[\gamma']\tp[-1-\gamma'+\delta']|T|\right), \\
\left|T^{\uLs\Ls} - \frac14T_{\Ls\uLs}\right| + \left|T^{\Ls\uLs} - \frac14T_{\uLs\Ls}\right| &\lesssim \epsilon\left(\tp[-1+\delta']|\slashed{T}| + \tm[\gamma']\tp[-1-\gamma'+\delta']|T|\right), \\
\left|T^{\Bs{i}\Bs{j}} - T_{\Bs{i}\Bs{j}}\right|  &\lesssim \epsilon\left(\tp[-1+\delta']|\slashed{T}| + \tm[\gamma']\tp[-1-\gamma'+\delta']|T|\right), \\
\left|T^{\Ls\Bs{j}} + \frac12 T_{\uLs\Bs{j}}\right| + \left|T^{\Bs{j}\Ls} + \frac12 T_{\Bs{j}\uLs}\right| &\lesssim \epsilon\tp[-1+\delta']|T|, \\
\left|T^{\Ls\Ls} - \frac14 T_{\uLs\uLs}\right|  &\lesssim \epsilon\tp[-1+\delta']|T|
\end{align}
\end{subequations}
\end{Lemma}
\begin{proof}
This almost entirely follows from equation \eqref{RMetric}. As an example, we prove our result for the first term on the left hand side of equation \eqref{ExampleRaised}. We first rewrite
\begin{equation}
T^{\uLs\Bs{j}} = \sum_{\substack{ X,Y \in \mcU}} g^{\uLs X}T_{XY}g^{Y\Bs{j}}
\end{equation}
If $X = \Ls$ and $Y = \Bs{j}$, we have the term which is subtracted off plus an error term which is directly bounded by the first term on the right hand side. If $X = \Ls$ and $Y = \Ls$ or $\Bs{i}$, we likewise have something bounded by the first term on the right. If $X = \Ls$ and $Y = \uLs$, we have a term like $g^{\uLs\Bs{j}}$, which has our better decay norm.
If $X \neq \Ls$, we likewise have either $g^{\uLs\uLs}$ or $g^{\uLs\Bs{i}}$, both of which have our better decay norms. Other component estimates follow similarly.
\end{proof}

Now we define a vector which will be useful in the energy estimate: 
\begin{equation}
\Lt = \nabla \us,
\end{equation}
the normal vector to surfaces of constant $\us$. We note that $\Lt$ is very close to a scalar multiple of $L$, in the sense that
\[
g_{\Lt\Ls}, g_{\Lt S_j^*} = 0,
\]
which is a restatement of the relations $\Ls(\us), \Bs{j}(\us) = 0$. We can say in particular that
\[
\Lt^{\uLs} \lesssim \epsilon\tm[\gamma']\tp[-1-\gamma'].
\]
This will be useful later, as we can bound error terms from the metric using an integrated $L^\infty$ estimate, at the expense of requiring more derivatives of the function in the energy.

